Token-Driven GammaTune: Adaptive Calibration for Enhanced Speculative Decoding

Speculative decoding accelerates large language model (LLM) inference by using a smaller draft model to propose tokens, which are then verified by a larger target model. However, selecting an optimal speculation length is critical for maximizing speedup while minimizing wasted computation. We introduce \textit{GammaTune} and \textit{GammaTune+}, training-free adaptive algorithms that dynamically adjust speculation length based on token acceptance rates using a heuristic-based switching mechanism. Evaluated on SpecBench across multiple tasks and model pairs, our method outperforms other heuristic-based approaches and fixed-length speculative decoding, achieving an average speedup of 15\% ($\pm$5\%) with \textit{GammaTune} and 16\% ($\pm$3\%) with \textit{GammaTune+}, while reducing performance variance. This makes \textit{GammaTune} a robust and efficient solution for real-world deployment.

==> figures/result_throughput.tex <==
% \documentclass{article}
% \usepackage{graphicx}
% \usepackage{subcaption}

% \begin{document}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/images/vicuna-13b-v1.5_vicuna-160m_mean.png}
        \caption{Vicuna-13B/Vicuna-160M}
        \label{fig:sub1}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/images/vicuna-7b-v1.5_vicuna-68m_mean.png}
        \caption{Vicuna-7B/Vicuna-68M}
        \label{fig:sub2}
    \end{subfigure}
    
    \vspace{1em}
    
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/images/vicuna-13b-v1.5_vicuna-160m_max.png}
    %     \caption{Max throughput (tokens/sec) for the Vicuna-13B/Vicuna-160M}
    %     \label{fig:sub3}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/images/vicuna-7b-v1.5_vicuna-68m_max.png}
    %     \caption{Max throughput (tokens/sec) for the Vicuna-7B/Vicuna-68M}
    %     \label{fig:sub4}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/images/Llama-3.1-70B-Instruct_Llama-3.1-8B-Instruct_mean.png}
        \caption{Llama-70B-Instruct/Llama-8B-Instruct}
        \label{fig:sub3}
    \end{subfigure}

    \caption{Comparison of the \textbf{average throughput} (tokens/sec) across three different model pairs using various speculative decoding methods. Error bars indicate standard deviations.}

    \label{fig:vicuna_results}
\end{figure}

% \end{document}


==> figures/results_acceptance.tex <==
% \documentclass{article}
% \usepackage{graphicx}
% \usepackage{subcaption}

% \begin{document}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/images/vicuna-13b-v1.5_vicuna-160m_acceptance_rate.png}
        \caption{Vicuna-13B/Vicuna-160M}
        \label{fig:sub1}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/images/vicuna-7b-v1.5_vicuna-68m_acceptance_rate.png}
        \caption{Vicuna-7B/Vicuna-68M}
        \label{fig:sub2}
    \end{subfigure}
    
    \vspace{1em}
    
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/images/vicuna-13b-v1.5_vicuna-160m_max.png}
    %     \caption{Max throughput (tokens/sec) for the Vicuna-13B/Vicuna-160M}
    %     \label{fig:sub3}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/images/vicuna-7b-v1.5_vicuna-68m_max.png}
    %     \caption{Max throughput (tokens/sec) for the Vicuna-7B/Vicuna-68M}
    %     \label{fig:sub4}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/images/Llama-3.1-70B-Instruct_Llama-3.1-8B-Instruct_acceptance_rate.png}
        \caption{Llama-70B-Instruct/Llama-8B-Instruct}
        \label{fig:sub3}
    \end{subfigure}

    \caption{Comparison of the \textbf{average acceptance rate} for three different model pairs, contrasting Speculative Decoding with optimal length and GammaTune across a range of initial speculation lengths. Error bars for GammaTune represent the standard deviation of the average acceptance rate over the different initial speculation lengths.}

    \label{fig:vicuna_results}
\end{figure}

% \end{document}


==> figures/results_gamma.tex <==
% \documentclass{article}
% \usepackage{graphicx}
% \usepackage{subcaption}

% \begin{document}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/images/vicuna-13b-v1.5_vicuna-160m_average_gamma.png}
        \caption{Vicuna-13B/Vicuna-160M}
        \label{fig:sub1}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/images/vicuna-7b-v1.5_vicuna-68m_average_gamma.png}
        \caption{Vicuna-7B/Vicuna-68M}
        \label{fig:sub2}
    \end{subfigure}
    
    \vspace{1em}
    
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/images/vicuna-13b-v1.5_vicuna-160m_max.png}
    %     \caption{Max throughput (tokens/sec) for the Vicuna-13B/Vicuna-160M}
    %     \label{fig:sub3}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/images/vicuna-7b-v1.5_vicuna-68m_max.png}
    %     \caption{Max throughput (tokens/sec) for the Vicuna-7B/Vicuna-68M}
    %     \label{fig:sub4}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/images/Llama-3.1-70B-Instruct_Llama-3.1-8B-Instruct_average_gamma.png}
        \caption{Llama-70B-Instruct/Llama-8B-Instruct}
        \label{fig:sub3}
    \end{subfigure}

    \caption{Comparison of the \textbf{average speculation length $\gamma$} for three different model pairs, contrasting Speculative Decoding with optimal length (fixed) and GammaTune across a range of initial speculation lengths. Error bars for GammaTune represent the standard deviation of the average speculation length $\gamma$ over the different initial speculation lengths.}

    \label{fig:vicuna_results}
\end{figure}

% \end{document}

